Level Lines of Gaussian Free Field I: Zero-Boundary GFF

Let $h$ be an instance of Gaussian Free Field in a planar domain. We study level lines of $h$ starting from boundary points. We show that the level lines are random continuous curves which are variants of SLE$_4$ path. We show that the level lines with different heights satisfy the same monotonicity behavior as the level lines of smooth functions. We prove that the time-reversal of the level line coincides with the level line of $-h$. This implies that the time-reversal of SLE$_4(\underline{\rho})$ process is still an SLE$_4(\underline{\rho})$ process. We prove that the level lines satisfy "target-independent" property. We also discuss the relation between Gaussian Free Field and CLE$_4$.

==> tex/boundary_levellines_intersecting_reversibility_leftover1.tex <==
We start by the generalizations of previous conclusions in the non-boundary-intersecting case to the case when the level lines can hit the boundary.

\begin{figure}[ht!]
\begin{subfigure}[b]{0.5\textwidth}
\begin{center}
\includegraphics[width=0.6\textwidth]{figures/boundary_levellines_case2_intersecting}
\end{center}
\caption{The boundary value of the field in Lemma \ref{lem::boundary_levellines_case2_intersecting}.}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\begin{center}\includegraphics[width=0.6\textwidth]{figures/boundary_levellines_case3_intersecting}
\end{center}
\caption{The boundary value of the field in Lemma \ref{lem::boundary_levellines_case3_intersecting}.}
\end{subfigure}
\caption{\label{fig::boundary_levellines_case23_intersecting} The boundary values of the fields in Lemma \ref{lem::boundary_levellines_case2_intersecting} and Lemma \ref{lem::boundary_levellines_case3_intersecting}.}
\end{figure}


\begin{lemma}\label{lem::boundary_levellines_case2_intersecting}[Generalization of Lemma \ref{lem::boundary_levellines_deterministic_case2}]
Suppose that $h$ is a $\GFF$ on $\T$. Assume that the boundary value of $h$ is piecewise constant, changes only finitely many times, and is
\[\begin{array}{ll}
\text{at most } -\lambda \text{ to the left of } z_0 \text{ on } \partial_U\T, & \text{at least } \lambda \text{ to the right of } z_0 \text{ on } \partial_U\T, \\
\text{at most } -\lambda \text{ to the left of } 0 \text{ on } \partial_L\T, & \text{greater than } -\lambda \text{ to the right of } 0 \text{ on } \partial_L\T.
\end{array}\]
See Figure \ref{fig::boundary_levellines_case23_intersecting}(a).
Let $\gamma$ be the level line of $h$ starting from 0 targeted at $z_0$. Then $\gamma$ almost surely hits $\partial_U\T$ at $z_0$ without otherwise hitting $\partial_U\T$.
\end{lemma}

\begin{proof}
We prove the conclusion by induction on the number of changes in $(0,\infty)$ on $\partial_L\T$. Suppose that
\[0=x_1<x_2<\cdots<x_n<x_{n+1}=\infty,\]
and that the boundary value of $h$ on $(x_j,x_{j+1})$ is $b_j>-\lambda$ for $j=1,...,n$. Lemma \ref{lem::boundary_levellines_continuity_tworight_forcepoints_generalization_1} implies that the conclusion holds for $n=1$. Suppose that the conclusion holds for $n\le m$ for some $m\ge 1$ and we will prove that the conclusion also holds for $n=m+1$. Let $\tau$ be the first time that $\gamma$ hits $[x_2,\infty]$ and set $\tau=\infty$ if $\gamma$ hits $\partial_U\T$ before hits $[x_2,\infty)$.

If $\tau=\infty$, then the law of $\gamma$ is absolutely continuous with respect to the level line of the GFF on $\T$ whose boundary value is consistent with $h$ outside $(0,\infty)$ and is $b_1$ on $(0,\infty)$. Therefore the conclusion holds by Lemma \ref{lem::boundary_levellines_continuity_tworight_forcepoints_generalization_1}. In the following, we assume that $\tau<\infty$. Define $C$ to be the connected component of $\T\setminus\gamma[0,\tau]$ that has $z_0$ on the boundary and let $\psi$ be the conformal map from $C$ onto $\T$ htat sends $\gamma(\tau)$ to 0, $+\infty$ to $+\infty$, and $z_0$ to $z_0$. Then, given $\gamma[0,\tau]$, the curve $\psi(\gamma|_C)$ is the level line of the GFF on $\T$ whose boundary value changes at most $m$ times on $(0,\infty)$. Thus the conclusion holds by induction hypothesis.
\end{proof}

\begin{lemma}\label{lem::boundary_levellines_case3_intersecting}[Generalization of Lemma \ref{lem::boundary_levellines_deterministic_case3}]
Suppose that $h$ is a $\GFF$ on $\T$. Assume that the boundary value of $h$ is piecewise constant, changes only finitely many times, and is between $-\lambda$ and $+\lambda$ in $[z_0,z_1]$ and is
\[\begin{array}{ll}
\text{at most } -\lambda \text{ to the left of } z_0 \text{ on } \partial_U\T, & \text{at least } \lambda \text{ to the right of } z_1 \text{ on } \partial_U\T, \\
\text{at most } -\lambda \text{ to the left of } 0 \text{ on } \partial_L\T, & \text{greater than } -\lambda \text{ to the right of } 0 \text{ on } \partial_L\T.
\end{array}\]
See Figure \ref{fig::boundary_levellines_case23_intersecting}(b).
Let $\gamma$ be the level line of $h$ starting from 0 targeted at $z_0$. Then $\gamma$ almost surely first hits $\partial_U\T$ in $[z_0,z_1]$ without otherwise hitting $\partial_U\T$.
\end{lemma}
\begin{proof} The conclusion can be proved by a similar proof of the proof of Lemma \ref{lem::boundary_levellines_case2_intersecting} where Lemma \ref{lem::boundary_levellines_continuity_tworight_forcepoints_generalization_1} needs to be replaced by Lemma \ref{lem::boundary_levellines_continuity_tworight_forcepoints_generalization_2}.
\end{proof}
\begin{figure}[ht!]
\begin{subfigure}[b]{0.3\textwidth}
\begin{center}
\includegraphics[width=\textwidth]{figures/boundary_levellines_coincide_intersecting_merge}
\end{center}
\caption{$\gamma$ has to hits $\gamma'[0,T']$ at $\gamma'(T')$ and merges with $\gamma'$ afterwards.}
\end{subfigure}
$\quad$
\begin{subfigure}[b]{0.3\textwidth}
\begin{center}\includegraphics[width=\textwidth]{figures/boundary_levellines_coincide_intersecting_left}
\end{center}
\caption{If $u>0$, $\gamma_u'[0,T']$ stays to the right of $\gamma$.}
\end{subfigure}
$\quad$
\begin{subfigure}[b]{0.3\textwidth}
\begin{center}\includegraphics[width=\textwidth]{figures/boundary_levellines__coincide_intersecting_right}
\end{center}
\caption{If $u<0$, $\gamma_u'[0,\tau']$ stays to the left of $\gamma$.}
\end{subfigure}
\caption{\label{fig::boundary_levellines__coincide_intersecting} The explanation of the behaviour of the paths in Lemma \ref{lem::boundary_levellines_coincide_intersecting} and Lemma \ref{lem::boundary_levellines_monotonicity_reverse_intersecting}}
\end{figure}


\begin{lemma}\label{lem::boundary_levellines_coincide_intersecting}[Generalization of Lemma \ref{lem::boundary_levellines_deterministic_nonintersecting_coincide}]
Suppose the same the setting as in Lemma \ref{lem::boundary_levellines_case2_intersecting}. Let $\gamma'$ be the level line of $-h$ starting from $z_0$ and define $T'$ to be the first time that $\gamma'$ hits $\partial_L\T$. Let $\gamma$ be the level line of $h$ starting from 0 targeted at $z_0$. Then, given $\gamma'[0,T']$, the level line $\gamma$ almost surely hits $\gamma'[0,T']$ at $\gamma'(T')$ and merges with $\gamma'$ afterwards. See Figure \ref{fig::boundary_levellines__coincide_intersecting}(a).
\end{lemma}

\begin{proof}
The conclusion can be proved by a similar proof as the proof of Lemma \ref{lem::boundary_levellines_deterministic_nonintersecting_coincide} where Lemma \ref{lem::boundary_levellines_deterministic_case2} needs to be replaced by Lemma \ref{lem::boundary_levellines_case2_intersecting}.
\end{proof}

\begin{lemma}\label{lem::boundary_levellines_monotonicity_reverse_intersecting}[Generalization of Proposition \ref{prop::boundary_levellines_nonintersecting_monotonicity_reverse}]
Suppose the same the setting as in Lemma \ref{lem::boundary_levellines_case2_intersecting}. Fix $u\in\R$ and let $\gamma'_u$ be the level line of $-h$ with height $u$ starting from $z_0$. Assume that $\gamma'_u$ does not hit its continuation threshold before reaches $\partial_L\T$ and define $T'$ to be the first time that $\gamma'_u$ hits $\partial_L\T$. Let $\gamma$ be the level line of $h$ starting from 0 targeted at $z_0$.
\begin{enumerate}
\item [(1)] If $u>0$, then $\gamma'_u[0,T']$ almost surely stays to the right of $\gamma$, see Figure \ref{fig::boundary_levellines__coincide_intersecting}(b).
\item [(2)] If $u<0$, then, for any $\gamma_u'$-stopping time $\tau'$ that is strictly before $T'$, we have that $\gamma'_u[0,\tau']$ stays to the left of $\gamma$, see Figure \ref{fig::boundary_levellines__coincide_intersecting}(c).
\end{enumerate}
\end{lemma}
\begin{proof}
The conclusion can be proved by a similar proof as the proof of Proposition \ref{prop::boundary_levellines_nonintersecting_monotonicity_reverse} where Lemma \ref{lem::boundary_levellines_deterministic_case3} needs to be replaced by Lemma \ref{lem::boundary_levellines_case3_intersecting}.
\end{proof}
\begin{figure}[ht!]
\begin{subfigure}[b]{0.5\textwidth}
\begin{center}
\includegraphics[width=0.6\textwidth]{figures/boundary_levellines_monotonicity_intersecting_1}
\end{center}
\caption{The boundary value of the field in Lemma \ref{lem::boundary_levellines_monotonicity_intersecting}.}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\begin{center}\includegraphics[width=0.6\textwidth]{figures/boundary_levellines_monotonicity_intersecting_2}
\end{center}
\caption{The level line $\gamma$ stays to the right of $\gamma'_{-u}$.}
\end{subfigure}
\caption{\label{fig::boundary_levellines_monotonicity_intersecting} The explanation of the behaviour of the paths in the proof of Lemma \ref{lem::boundary_levellines_monotonicity_intersecting}.}
\end{figure}

\begin{lemma}\label{lem::boundary_levellines_monotonicity_intersecting}[Generalization of Proposition \ref{prop::boundary_levellines_nonintersecting_monotonicity}]
Suppose that $h$ is a $\GFF$ on $\T$. Fix $u>0$ and assume that the boundary value of $h$ is piecewise constant, changes only finitely many times, and is at most $-\lambda-u$ to the left of $0$ on $\partial_L\T$ and is greater than $-\lambda$ and at least $\lambda-u$ to the right of $0$ on $\partial_L\T$, see Figure \ref{fig::boundary_levellines_monotonicity_intersecting}(a). Let $\gamma$ be the level line of $h$ starting from 0 and $\gamma_u$ be the level line of $h$ with height $u$ starting from 0. Then $\gamma_u$ almost surely stays to the left of $\gamma$ up to the first time that they accumulate in $\partial_U\T$. We emphasize that there is no restriction for the boundary value of $h$ on $\partial_U\T$.
\end{lemma}
\begin{proof}
From the proof of Proposition \ref{prop::boundary_levellines_nonintersecting_monotonicity}, we know that we may assume that the boundary value of $h$ on $\partial_U\T$ is $-a'$ on $(-\infty,z_0)$ and is $b'$ on $(z_0,\infty)$. Assume that $a',b'$ are very large. Let $\gamma'_{-u}$ be the level line of $-h$ with height $-u$ starting from $z_0$ targeted at 0. We have the following two observations.
\begin{enumerate}
\item [(a)] From Proposition \ref{prop::boundary_levellines_deterministic_nonintersecting_coincide} and Remark \ref{rem::boundary_levellines_deterministic_nonintersecting_coincide}, we know that $\gamma'_{-u}$ and $\gamma_u$ are equal.
\item [(b)] From Lemma \ref{lem::boundary_levellines_monotonicity_reverse_intersecting}, we know that $\gamma'_{-u}[0,\tau']$ stays to the left of $\gamma$ for any $\gamma'_{-u}$-stopping time $\tau'$ that is strictly before $\gamma'_{-u}$ hits $\partial_L\T$. Note that $\gamma'_{-u}$ accumulates at $\partial_L\T$ at $0$ without otherwise hitting $\partial_L\T$. Thus $\gamma'_{-u}$ stays to the left of $\gamma$. See Figure \ref{fig::boundary_levellines_monotonicity_intersecting}(b).
\end{enumerate}
Combining these two facts, we know that $\gamma_u$ stays to the left of $\gamma$.
\end{proof}

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.3\textwidth]{figures/chordal_sle_reversibility_onlyright}
\end{center}
\caption{\label{fig::chordal_sle_reversibility_onlyright} The explanation of the behaviour of the paths in the proof of Proposition \ref{prop::chordal_sle_reversibility_onlyright}.}
\end{figure}


\begin{proposition}\label{prop::chordal_sle_reversibility_onlyright}
Fix $0=x_1<x_2<\cdots<x_n<x_{n+1}=\infty$. Suppose that $h$ is a $\GFF$ on $\HH$ whose boundary value is $-a$ on $\R_-$ and is $b_j$ on $(x_j,x_{j+1})$ for $j=1,...,n$. Assume that
\[a\ge \lambda,\quad b_j>-\lambda, \quad \text{for } j=1,...,n.\]
Let $\gamma$ be the level line of $h$ starting from 0 targeted at $\infty$ and let $\gamma'$ be the level line of $-h$ starting from $\infty$ targeted at 0. Then $\gamma'$ and $\gamma$ are equal almost surely.
\end{proposition}
\begin{proof}
We prove by induction on $n$. Proposition \ref{prop::boundary_levellines_tworight} and Remark \ref{rem::boundary_levellines_tworight} imply that the conclusion holds for $n\le 2$. Assume that the conclusion holds for $n\le m$ for some $m\ge 2$, we will show that the conclusion holds for $n=m+1$. If all $b_j\ge \lambda$, then Proposition \ref{prop::boundary_levellines_deterministic_nonintersecting_coincide} and Remark \ref{rem::boundary_levellines_deterministic_nonintersecting_coincide} prove the conclusion. In the following, we assume that there exists some $b_j\in (-\lambda,\lambda)$.
\smallbreak
\textit{First}, we assume that $b_{n+1}\ge\lambda$. Define $n_0\le n$ to be the number so that $b_j\ge \lambda$ for $j>n_0$ and $b_{n_0}\in (-\lambda,\lambda)$. Set $\tilde{u}=\lambda+b_{n_0}\in (0,2\lambda)$. Let $\tilde{\gamma}'$ be the level line of $-h$ with height $\tilde{u}$ starting from $\infty$ targeted at $x_{n_0+1}$. We summarize the relations between $\gamma,\gamma'$ and $\tilde{\gamma}'$ as follows.
\begin{enumerate}
\item [(a)] $\tilde{\gamma}'$ is continuous up to and including the continuation threshold. Define $C$ to be the connected component of $\HH\setminus\tilde{\gamma}'$ that has $\R_-$ on the boundary.
\item [(b)] By Lemma \ref{lem::boundary_levellines_monotonicity_intersecting}, we know that $\gamma'$ stays to the left of $\tilde{\gamma}'$; moreover, given $\tilde{\gamma}'$, the conditional law of $\gamma'$ is the same as the level line of $-h|_C$ starting from $\infty$.
\item [(c)] By Lemma \ref{lem::boundary_levellines_monotonicity_reverse_intersecting}, we know that $\gamma$ stays to the left of $\tilde{\gamma}'$; moreover, given $\tilde{\gamma}'$, the conditional law of $\gamma$ is the same as the level line of $h|_C$ starting from 0.
\end{enumerate}
Given $\tilde{\gamma}'$, combining the above three facts and noting that the number of changes of $h|_C$ is at most $n_0\le m$, we have that $\gamma'$ and $\gamma$ are equal by induction hypothesis. This implies the conclusion.
\smallbreak
\textit{Next}, we assume that $b_{n+1}\in (-\lambda,\lambda)$. {\large{\color{red}TBA}}
\begin{comment}Let $\tilde{h}$ be the GFF on $\HH$ whose boundary value is consistent with $h$ outside $(x_{n+1},\infty)$ and is $\lambda$ on $(x_{n+1},\infty)$. Let $\gamma$ be the level line of $\tilde{h}$ starting from 0 targeted at $\infty$ and $\gamma'$ be the level line of $-h$ starting from $\infty$ targeted at 0. Let $\tilde{\gamma}'$ be the level line of $\tilde{h}$ with height $\tilde{u}=\lambda+b_{n+1}\in (0,2\lambda)$ starting from $\infty$ targeted at $x_{n+1}$. We summarize the relations between $\gamma,\gamma'$ and $\tilde{\gamma}'$ as follows.
\begin{enumerate}
\item [(a)] By the first step, we know that $\gamma'$ and $\gamma$ are equal.
\item [(b)] $\tilde{\gamma}'$ is continuous up to and including the continuation threshold. Define $C$ to the connected component of $\HH\setminus\tilde{\gamma}'$ that has $\R_-$ on the boundary.
\item [(c)] By Lemma \ref{lem::boundary_levellines_monotonicity_intersecting}, we know that $\gamma'$ stays to the left of $\tilde{\gamma}'$; moreover, given $\tilde{\gamma}'$, the conditional law of $\gamma'$ is the same as the level line of $-\tilde{h}|_C$ starting from $\infty$.
\item [(d)] By Lemma \ref{lem::boundary_levellines_monotonicity_reverse_intersecting}, we know that $\gamma$ stays to the left of $\tilde{\gamma}'$; moreover, given $\tilde{\gamma}'$, the conditional law of $\gamma$ is the same as the level line of $\tilde{h}|_C$ starting from 0.
\end{enumerate}
Combining these four facts, we know that $\gamma'$ and $\gamma$ are equal given $\tilde{\gamma}'$. This implies the conclusion.
\end{comment}
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm::sle_chordal_reversibility}]
\large{\color{red}TBA}
\end{proof}


==> tex/boundary_levellines_intersecting_reversibility_leftover2.tex <==
In this section, we work in $\T$. We summarize the notations in the following remark.
\begin{remark}\label{rem::boundary_levellines_reversibility_notations}
Suppose that
\[\underline{z}^L=(z_1^L=z_0>z_2^L>\cdots>z^L_{l'}>z^L_{l'+1}=-\infty)\]
is a sequence of points to the left of $z_0$ on $\partial_U\T$; that
\[\underline{z}^R=(z_1^R=z_0<z_2^R<\cdots<z^R_{r'}<z^R_{r'+1}=+\infty)\]
is a sequence of points to the right of $z_0$ on $\partial_U\T$; that
\[\underline{x}^L=(x_1^L=0>x_2^L>\cdots>x^L_{l}>x^L_{l+1}=-\infty)\]
is a sequence of points to the left of $0$ on $\partial_L\T$; and that
\[\underline{x}^R=(x_1^R=0<x_2^R<\cdots<x^R_{r}<x^R_{r+1}=+\infty)\]
is a sequence of points to the right of $0$ on $\partial_L\T$. See Figure \ref{fig::boundary_levellines_reversibility_notations}.

Suppose that $h$ is a GFF on $\T$ whose boundary value is
\[\begin{array}{llllllllll}
-a'_j&\text{on}&(z^L_{j+1},z^L_j),&\text{for}& j=1,...,l';&
b'_j&\text{on}&(z^R_{j},z^R_{j+1}),&\text{for}& j=1,...,r';\\
-a_j&\text{on}&(x^L_{j+1},x^L_j),&\text{for}& j=1,...,l;&
b_j&\text{on}&(x^R_{j},x^R_{j+1}),&\text{for}& j=1,...,r.
\end{array}\]
Let $\gamma$ be the level line of $h$ starting from 0 targeted at $z_0$ and $\gamma'$ be the level line of $-h$ starting from $z_0$ targeted at $0$.
\end{remark}

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.355\textwidth]{figures/boundary_levellines_reversibility_notations}
\end{center}
\caption{\label{fig::boundary_levellines_reversibility_notations} The explanation of the notations Remark \ref{rem::boundary_levellines_reversibility_notations}.}
\end{figure}

\begin{lemma}\label{lem::boundary_levellines_reversibility_rightbottom}
Suppose the same notations as in Remark \ref{rem::boundary_levellines_reversibility_notations}. Assume that
\[\begin{array}{llllll}
a'_j\ge\lambda &\text{for}& j=1,...,l';&b'_j\ge\lambda &\text{for}& j=1,...,r';\\
a_j\ge\lambda &\text{for}& j=1,...,l;&b_j>-\lambda&\text{for}& j=1,...,r.
\end{array}\]
Then almost surely $\gamma'$ and $\gamma$ are equal.
\end{lemma}
\begin{proof}
We prove by induction on $r$. 
\smallbreak
\textit{First}, we show that the conclusion holds for $r=1$. In this part, we suppose $r=1$. By Proposition \ref{prop::boundary_levellines_tworight} and Remark \ref{rem::boundary_levellines_tworight}, we know that the conclusion holds when $r'=1$. Suppose that $r'\ge 2$. For any $\eps>0$ define $\T_{\eps}$ to be the open set obtained by removing from $\T$ all points that are within distance $\eps$ of $[z_2^R,\infty)$ on $\partial_U\T$. Define $E_{\eps}$ to be the event that the distance between $\gamma\cup\gamma'$ and $[z_2^R,\infty)$ is at least $\eps$. Let $\tilde{h}$ be a GFF on $\T$  whose boundary value is consistent with $h$ except on $(z_0,\infty)$ and is $b_1'$ on $(z_0,\infty)$ on $\partial_U\T$. Let $\tilde{\gamma}$ be the level line of $\tilde{h}$ starting from 0 targeted at $z_0$ and let $\tilde{\gamma}'$ be the level line of $-\tilde{h}$ starting from $z_0$ targeted at 0. Then we have the following facts.
\begin{enumerate}
\item [(a)] By Proposition \ref{prop::boundary_levellines_tworight} and Remark \ref{rem::boundary_levellines_tworight}, we have that $\tilde{\gamma}'$ and $\tilde{\gamma}$ are equal.
\item [(b)] The law of $h$ restricted to $\T_{\eps}$ is absolutely continuous with respect to the law of $\tilde{h}$ restricted $\T_{\eps}$.
\end{enumerate}
Combining these two facts, we know that, on $E_{\eps}$, the curves $\gamma'$ and $\gamma$ are equal. Since that the boundary value on $(z_2^R,\infty)$ is at least $\lambda$, the union $\gamma\cup\gamma'$ has positive distance from $(z_2^R,\infty)$ almost surely. Therefore $\PP[E_{\eps}]\to 1$ as $\eps\to 0$, this implies the conclusion.
\smallbreak
\textit{Next}, we assume that the conclusion holds for $r\le m$ for some $m\ge 1$. We will prove that the conclusion also holds for $r=m+1$. We divide the situation into three cases according to the value of $b_m$ and $b_{m+1}$: Case 1. $b_{m+1}\ge \lambda$; Case 2. $b_{m+1}$
\smallbreak
Case 1. Assume that $b_{m+1}\ge\lambda$. Define $\psi$ to be the conformal map from $\T$ onto $\T$ such that sends $0$ to $0$, $x_{m+1}^R$ to $+\infty$, and $z_0$ to $z_0$. By the induction hypothesis, we know that $\psi(\gamma')$ and $\psi(\gamma)$ are equal which implies that $\gamma'$ and $\gamma$ are equal.
\smallbreak
Case 2. Assume that $b_{m+1}\in (-\lambda,\lambda)$. Suppose that $\tilde{h}$ is a GFF on $\T$ whose boundary value is consistent with $h$ except on $(x_{m+1}^R,\infty)$ and is $\lambda$ on $(x_{m+1}^R,\infty)$ on $\partial_L\T$. Let $\tilde{\gamma}$ be the level line of $\tilde{h}$ starting from 0 targeted at $z_0$ and $\tilde{\gamma}'$ be the level line of $-\tilde{h}$ starting from $z_0$ targeted at 0. Set 
\end{proof}

\begin{figure}[ht!]
\begin{subfigure}[b]{0.5\textwidth}
\begin{center}
\includegraphics[width=0.71\textwidth]{figures/boundary_levellines_reversibility_rightbottom}
\end{center}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\begin{center}\includegraphics[width=0.71\textwidth]{figures/boundary_levellines_reversibility_rightbottom}
\end{center}
\caption{}
\end{subfigure}
\caption{\label{fig::boundary_levellines_reversibility_right} The explanation of the behaviour of the paths in Lemmas \ref{lem::boundary_levellines_reversibility_rightbottom} \ref{lem::boundary_levellines_reversibility_right}.}
\end{figure}

\begin{lemma}\label{lem::boundary_levellines_reversibility_right}
Suppose the same notations as in Remark \ref{rem::boundary_levellines_reversibility_notations}. Assume that
\[\begin{array}{llllll}
a'_j\ge\lambda &\text{for}& j=1,...,l';&b'_j>-\lambda &\text{for}& j=1,...,r';\\
a_j\ge\lambda &\text{for}& j=1,...,l;&b_j>-\lambda&\text{for}& j=1,...,r.
\end{array}\]
Then almost surely $\gamma'$ and $\gamma$ are equal.
\end{lemma}
\begin{proof}
{\color{red}TBA}
\end{proof}
\begin{lemma}\label{lem::boundary_levellines_reversibility_right_leftbottom}
Suppose the same notations as in Remark \ref{rem::boundary_levellines_reversibility_notations}. Assume that
\[\begin{array}{llllll}
a'_j\ge\lambda &\text{for}& j=1,...,l';&b'_j>-\lambda &\text{for}& j=1,...,r';\\
a_j>-\lambda &\text{for}& j=1,...,l;&b_j>-\lambda&\text{for}& j=1,...,r.
\end{array}\]
Then almost surely $\gamma'$ and $\gamma$ are equal.
\end{lemma}
\begin{proof}
{\color{red}TBA}
\end{proof}
\begin{lemma}\label{lem::boundary_levellines_reversibility_right_left}
Suppose the same notations as in Remark \ref{rem::boundary_levellines_reversibility_notations}. Assume that
\[\begin{array}{llllll}
a'_j>-\lambda &\text{for}& j=1,...,l';&b'_j>-\lambda &\text{for}& j=1,...,r';\\
a_j>-\lambda &\text{for}& j=1,...,l;&b_j>-\lambda&\text{for}& j=1,...,r.
\end{array}\]
Then almost surely $\gamma'$ and $\gamma$ are equal.
\end{lemma}
\begin{proof}
{\color{red}TBA}
\end{proof}
\begin{proof}[Proof of Theorem \ref{thm::sle_chordal_reversibility}]
{\color{red}TBA}
\end{proof}


==> tex/relation_previous_outline.tex <==
{\color{red}TBA}
\medbreak
\textbf{Acknowledgement}
